Joint Language Semantic and Structure Embedding for Knowledge Graph Completion

The task of completing knowledge triplets has broad downstream applications. Both structural and semantic information plays an important role in knowledge graph completion. Unlike previous approaches that rely on either the structures or semantics of the knowledge graphs, we propose to jointly embed the semantics in the natural language description of the knowledge triplets with their structure information. Our method embeds knowledge graphs for the completion task via fine-tuning pre-trained language models with respect to a probabilistic structured loss, where the forward pass of the language models captures semantics and the loss reconstructs structures. Our extensive experiments on a variety of knowledge graph benchmarks have demonstrated the state-of-the-art performance of our method. We also show that our method can significantly improve the performance in a low-resource regime, thanks to the better use of semantics. The code and datasets are available at https://github.com/pkusjh/LASS.

==> chap/miscs.tex <==

% Traditional approaches, such as TransE~\cite{TransE} and RotatE~\cite{RotateE}, focus on learning the structural patterns in the existing triplets to predict the missing pieces. For example, a composition pattern can be learned to predict the relation \texthrt{grandmother\_Of} based on two consecutive \texthrt{mother\_Of} relations. Besides the structure information, we have noticed that the semantic relatedness between entities and relations are critical to infer entities or relations with similar meanings. For example, if a relationship \texthrt{CEO\_Of} holds between two entities, \texthrt{employee\_Of} also holds. Some recent works~\cite{KGBERT,KB_NL_5,KB_NL_6} leverage the natural language description of entities and relations to predict such semantically relevant entities or relations, and lead to significant improvements. Therefore, an approach that can leverage both structural and semantic information of the KGs is expected.


\iffalse
\subsection{Related Models}
\label{sec:relatedmodel}
There are several key differences between our \method\ and KG-BERT~\cite{KGBERT}: (\expandafter{\romannumeral1}) \method\ reconstructs the structures of KGs via structure embedding, while KG-BERT does not; (\expandafter{\romannumeral2}) \method\ unifies the link prediction and triplet classification under the same architecture (see Sec.~\ref{sec:exp} for details), while KG-BERT designs different architectures for different tasks; (\expandafter{\romannumeral3}) \method\ works with two families of LMs, while KG-BERT only works with BERT$_{\rm BASE}$. \method\ is not particularly designed for BERT, shedding light on understanding the role of semantics in LMs for the KG completion.

TransE~\cite{TransE} treats the relation as a translation of the embeddings from the head to tail. Therefore $\mathbf{h} + \mathbf{r} \approx \mathbf{t}$ when \texthrt{(h, r, t)} holds. TransE designs a margin-based ranking loss based on the $l_2$ norm $\Vert \mathbf{h}+\mathbf{r}-\mathbf{t} \Vert_2^2$. The key differences between \method\ and TransE are: (\expandafter{\romannumeral1}) \method\ leverages the natural language semantics in LMs, while TransE does not; (\expandafter{\romannumeral2}) \method\ is a probabilistic structured loss, and is more computationally efficient and data-efficient compared to TransE. The main advantage of the probabilistic loss is that we eliminate the norm calculation that TransE requires to prevent the training process to trivially minimize its loss by increasing the embeddings of entities or relations. The ranking loss of TransE calculates the loss of some training examples as zeros, which will not contribute to the optimization procedure. Our probabilistic loss makes use of all the training examples. Besides, we introduce corrupted relations in the loss, which provides more flexibility in incorporating the KG structure.
\fi
